Supernova Host Galaxies in the Dark Energy Survey: I. Deep Coadds, Photometry, and Stellar Masses

The five-year Dark Energy Survey supernova programme (DES-SN) is one of the largest and deepest transient surveys to date in terms of volume and number of supernovae. Identifying and characterising the host galaxies of transients plays a key role in their classification, the study of their formation mechanisms, and the cosmological analyses. To derive accurate host galaxy properties, we create depth-optimised coadds using single-epoch DES-SN images that are selected based on sky and atmospheric conditions. For each of the five DES-SN seasons, a separate coadd is made from the other 4 seasons such that each SN has a corresponding deep coadd with no contaminating SN emission. The coadds reach limiting magnitudes of order $\sim 27$ in $g$-band, and have a much smaller magnitude uncertainty than the previous DES-SN host templates, particularly for faint objects. We present the resulting multi-band photometry of host galaxies for samples of spectroscopically confirmed type Ia (SNe Ia), core-collapse (CCSNe), and superluminous (SLSNe) as well as rapidly evolving transients (RETs) discovered by DES-SN. We derive host galaxy stellar masses and probabilistically compare stellar-mass distributions to samples from other surveys. We find that the DES spectroscopically confirmed sample of SNe Ia selects preferentially fewer high mass hosts at high redshift compared to other surveys, while at low redshift the distributions are consistent. DES CCSNe and SLSNe hosts are similar to other samples, while RET hosts are unlike the hosts of any other transients, although these differences have not been disentangled from selection effects.

==> corner_plots/mcmc_results.tex <==

\twocolumn
\section{}\label{app:fitparams}
The following tables show the results from the two-sample Bayesian fits as described in Section \ref{subsec:res_stats}. Loc, scale, and alpha correspond to the location (i.e. central mass), width, and skewness of the distributions respectively. Negative values in the difference parameters mean the DES sample (blue in Appendix C) has a lower value than the comparison sample (yellow in Appendix C).
\begin{table}
\caption{Results of the MCMC fits for comparing the stellar mass distributions for SNe Ia}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error \\
\midrule
DES SNe Ia AAT loc   & 11.083 & 0.037 &     0.001 \\
DES SNe Ia AAT scale &  1.462 & 0.036 &     0.001 \\
DES SNe Ia AAT alpha & -8.165 & 1.820 &     0.055 \\
PTF SNe Ia loc       & 11.140 & 0.030 &     0.001 \\
PTF SNe Ia scale     &  1.274 & 0.026 &     0.001 \\
PTF SNe Ia alpha     & -4.694 & 2.336 &     0.127 \\
\midrule
difference of locs   & -0.057 & 0.048 &     0.001 \\
difference of scales &  0.188 & 0.044 &     0.001 \\
difference of alphas & -3.471 & 2.957 &     0.136 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error \\
\midrule
DES SNe Ia AAT loc   & 11.085 & 0.037 &     0.001 \\
DES SNe Ia AAT scale &  1.463 & 0.036 &     0.001 \\
DES SNe Ia AAT alpha & -8.096 & 1.719 &     0.051 \\
PS1 SNe Ia loc       & 11.555 & 0.035 &     0.001 \\
PS1 SNe Ia scale     &  1.804 & 0.052 &     0.001 \\
PS1 SNe Ia alpha     & -5.740 & 0.864 &     0.019 \\
\midrule
difference of locs   & -0.470 & 0.050 &     0.001 \\
difference of scales & -0.341 & 0.063 &     0.001 \\
difference of alphas & -2.356 & 1.923 &     0.055 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error\\
\midrule
DES SNe Ia AAT loc   & 11.082 & 0.038 &     0.001 \\
DES SNe Ia AAT scale &  1.461 & 0.037 &     0.001 \\
DES SNe Ia AAT alpha & -8.253 & 2.009 &     0.077 \\
SNLS SNe Ia loc      & 11.152 & 0.020 &     0.001 \\
SNLS SNe Ia scale    &  1.549 & 0.030 &     0.001 \\
SNLS SNe Ia alpha    & -3.400 & 0.311 &     0.009 \\
\midrule

difference of locs   & -0.070 & 0.043 &     0.001 \\
difference of scales & -0.088 & 0.048 &     0.001 \\
difference of alphas & -4.854 & 2.052 &     0.079 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Results of the MCMC fits for comparing the stellar mass distrutions for CCSNe}

\begin{tabular}{lrrrrr}
\toprule
{} &    mean &    std &  mc\_error &\\
\midrule
DES CCSNe AAT loc   & 10.440 & 0.063 &     0.001 \\
DES CCSNe AAT scale &  1.371 & 0.066 &     0.001 \\
DES CCSNe AAT alpha & -7.000 & 3.575 &     0.129 \\
SDSS CCSNe loc      & 10.444 & 0.072 &     0.002 \\
SDSS CCSNe scale    &  1.606 & 0.060 &     0.001 \\
SDSS CCSNe alpha    & -4.291 & 2.068 &     0.103 \\
\midrule
difference of locs   & -0.004 & 0.093 &     0.002 \\
difference of scales & -0.235 & 0.089 &     0.002 \\
difference of alphas & -2.709 & 4.150 &     0.166 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Results of the MCMC fits for comparing the stellar mass distributions for RETs}
\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error \\
\midrule
DES RETs loc   &  9.738 & 0.288 &     0.019 \\
DES RETs scale &  0.714 & 0.077 &     0.004 \\
DES RETs alpha & -1.507 & 2.502 &     0.162 \\
PS1 RETs loc   &  8.749 & 0.294 &     0.016 \\
PS1 RETs scale &  0.495 & 0.225 &     0.012 \\
PS1 RETs alpha &  2.369 & 7.841 &     0.480 \\
\midrule

difference of locs   &  0.989 & 0.410 &     0.026 \\
difference of scales &  0.219 & 0.236 &     0.012 \\
difference of alphas & -3.876 & 8.453 &     0.526 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error & \\
\midrule
DES RETs loc        &  9.744 & 0.282 &     0.016 \\
DES RETs scale      &  0.715 & 0.075 &     0.003 \\
DES RETs alpha      & -1.778 & 2.877 &     0.155 \\
DES CCSNe AAT loc   & 10.444 & 0.066 &     0.002 \\
DES CCSNe AAT scale &  1.373 & 0.067 &     0.002 \\
DES CCSNe AAT alpha & -6.566 & 2.967 &     0.119 \\
\midrule
difference of locs   & -0.701 & 0.287 &     0.016 \\
difference of scales & -0.658 & 0.100 &     0.003 \\
difference of alphas &  4.788 & 4.165 &     0.211 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error & \\
\midrule
DES RETs loc         &  9.766 & 0.272 &     0.017 \\
DES RETs scale       &  0.717 & 0.076 &     0.003 \\
DES RETs alpha       & -1.572 & 2.216 &     0.123 \\
DES SNe Ia AAT loc   & 11.084 & 0.037 &     0.001 \\
DES SNe Ia AAT scale &  1.462 & 0.037 &     0.001 \\
DES SNe Ia AAT alpha & -8.135 & 1.869 &     0.063 \\
\midrule

difference of locs   & -1.318 & 0.274 &     0.017 \\
difference of scales & -0.745 & 0.084 &     0.003 \\
difference of alphas &  6.563 & 2.923 &     0.140 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error  \\
\midrule
DES RETs loc    &  9.745 & 0.288 &     0.019 \\
DES RETs scale  &  0.716 & 0.078 &     0.003 \\
DES RETs alpha  & -1.367 & 1.953 &     0.113 \\
DES SLSNe loc   &  8.376 & 0.608 &     0.036 \\
DES SLSNe scale &  0.679 & 0.171 &     0.007 \\
DES SLSNe alpha & -1.288 & 5.700 &     0.332 \\

\midrule
difference of locs   &  1.369 & 0.689 &     0.043 \\
difference of scales &  0.037 & 0.187 &     0.008 \\
difference of alphas & -0.078 & 6.024 &     0.355 \\
\bottomrule
\end{tabular}

\end{table}

\begin{table}
\caption{Results of the MCMC fits for comparing the stellar mass distributions for SLSNe}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error\\
\midrule
DES SLSNe loc   &   8.256 & 0.552 &     0.028 \\
DES SLSNe scale &   0.668 & 0.166 &     0.007 \\
DES SLSNe alpha &   0.046 & 5.147 &     0.282 \\
PTF SLSNe loc   &  10.655 & 0.034 &     0.001 \\
PTF SLSNe scale &   1.579 & 0.105 &     0.002 \\
PTF SLSNe alpha & -11.862 & 3.757 &     0.128 \\
\midrule

difference of locs   & -2.399 & 0.553 &     0.028 \\
difference of scales & -0.912 & 0.195 &     0.008 \\
difference of alphas & 11.908 & 6.388 &     0.305 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error \\
\midrule
DES SLSNe loc   & 8.229 & 0.567 &     0.035 \\
DES SLSNe scale & 0.678 & 0.163 &     0.007 \\
DES SLSNe alpha & 0.085 & 5.387 &     0.384 \\
PS+ SLSNe loc   & 7.164 & 0.109 &     0.004 \\
PS+ SLSNe scale & 0.718 & 0.054 &     0.002 \\
PS+ SLSNe alpha & 5.295 & 3.428 &     0.148 \\
\midrule

difference of locs   &  1.064 & 0.581 &     0.036 \\
difference of scales & -0.040 & 0.172 &     0.007 \\
difference of alphas & -5.210 & 6.240 &     0.400 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrr}
\toprule
{} &   mean &    std &  mc\_error \\
\midrule
DES SLSNe loc       &  8.304 & 0.578 &     0.031 \\
DES SLSNe scale     &  0.671 & 0.168 &     0.007 \\
DES SLSNe alpha     & -0.988 & 5.697 &     0.280 \\
DES CCSNe AAT loc   & 10.444 & 0.065 &     0.002 \\
DES CCSNe AAT scale &  1.372 & 0.067 &     0.002 \\
DES CCSNe AAT alpha & -6.844 & 3.336 &     0.144 \\
\midrule
difference of locs   & -2.140 & 0.581 &     0.031 \\
difference of scales & -0.701 & 0.184 &     0.007 \\
difference of alphas &  5.856 & 6.687 &     0.318 \\
\bottomrule
\end{tabular}
\end{table}


==> stacktable.tex <==

\begin{longtable}{lllllllr}
\toprule
 Field & Band & MY & $\tau_{\textrm{eff}}$ Cut & PSF Cut & $N_{\textrm{exp}}$ & $t_{\textrm{exp;tot}}$ &  $m_{\textrm{lim}}$ \\
\midrule
\endhead
\midrule
\endfoot

\bottomrule
\endlastfoot
 SN-E1 &    g &  1 &                      0.26 &     2.4 &                 70 &                    3.4 &               25.44 \\
 SN-E1 &    g &  2 &                      0.26 &     2.4 &                 48 &                   2.33 &               24.55 \\
 SN-E1 &    g &  3 &                      0.26 &     2.4 &                 54 &                   2.62 &               25.46 \\
 SN-E1 &    g &  4 &                      0.26 &     2.4 &                 52 &                   2.53 &               25.41 \\
 SN-E1 &    g &  5 &                      0.26 &     2.4 &                 60 &                   2.92 &               25.44 \\
 SN-E1 &    r &  1 &                       0.2 &     2.2 &                 90 &                   3.75 &               25.51 \\
 SN-E1 &    r &  2 &                       0.2 &     2.2 &                 69 &                   2.88 &               25.05 \\
 SN-E1 &    r &  3 &                       0.2 &     2.2 &                 69 &                   2.88 &               25.52 \\
 SN-E1 &    r &  4 &                       0.2 &     2.2 &                 63 &                   2.62 &               25.42 \\
 SN-E1 &    r &  5 &                       0.2 &     2.2 &                 73 &                   3.04 &               25.41 \\
 SN-E1 &    i &  1 &                       0.2 &     2.2 &                 95 &                   5.28 &               25.43 \\
 SN-E1 &    i &  2 &                       0.2 &     2.2 &                 74 &                   4.11 &               25.24 \\
 SN-E1 &    i &  3 &                       0.2 &     2.2 &                 72 &                    4.0 &               25.40 \\
 SN-E1 &    i &  4 &                       0.2 &     2.2 &                 68 &                   3.78 &               25.36 \\
 SN-E1 &    i &  5 &                       0.2 &     2.2 &                 75 &                   4.17 &               25.41 \\
 SN-E1 &    z &  1 &                       0.3 &     2.2 &                171 &                    9.5 &               25.23 \\
 SN-E1 &    z &  2 &                       0.3 &     2.2 &                132 &                   7.33 &               25.05 \\
 SN-E1 &    z &  3 &                       0.3 &     2.2 &                130 &                   7.22 &               25.24 \\
 SN-E1 &    z &  4 &                       0.3 &     2.2 &                125 &                   6.94 &               25.17 \\
 SN-E1 &    z &  5 &                       0.3 &     2.2 &                138 &                   7.67 &               25.22 \\
 \end{longtable}

